Bunched LPCNet2: Efficient Neural Vocoders Covering Devices from Cloud to Edge

Text-to-Speech (TTS) services that run on edge devices have many advantages compared to cloud TTS, e.g., latency and privacy issues. However, neural vocoders with a low complexity and small model footprint inevitably generate annoying sounds. This study proposes a Bunched LPCNet2, an improved LPCNet architecture that provides highly efficient performance in high-quality for cloud servers and in a low-complexity for low-resource edge devices. Single logistic distribution achieves computational efficiency, and insightful tricks reduce the model footprint while maintaining speech quality. A DualRate architecture, which generates a lower sampling rate from a prosody model, is also proposed to reduce maintenance costs. The experiments demonstrate that Bunched LPCNet2 generates satisfactory speech quality with a model footprint of 1.1MB while operating faster than real-time on a RPi 3B. Our audio samples are available at https://srtts.github.io/bunchedLPCNet2.

==> BunchedLPCNet2_INTERSPEECH2022 (Version 4313)/bunched_lpcnet.tex <==
\label{section:bunched}



In our previous study~\cite{bunched}, Sample Bunching was proposed as depicted in Figure~\ref{fig:bunched}. It allows LPCNet to generate multiple samples per GRU inference. Bit Bunching was also proposed to reduce the computations in the DualFC and softmax layers by splitting the output bits in two: the higher 7 bits for coarse prediction and lower 4 bits for fine correction.

\begin{figure}[t]
\centering
\includegraphics[width=0.40\textwidth]{figures/bunched2.pdf}
\caption{Bunched LPCNet overview}
\label{fig:bunched}
\end{figure}

Bunching techniques are sufficiently efficient for application in mobile devices, e.g., a smartphone. However, several limitations exist for further reducing computations for low-resource devices. (1) Sample Bunching reduces the computations of GRUs by $1/S$ times. This indicates that as the bunch size $S$ increases, the amount of computational reduction is saturated, especially where $S>4$. (2) Reducing the number of $\text{GRU}_{\text{A}}$ units with Bunching techniques significantly degrades the speech quality. Note that $\text{GRU}_{\text{A}}$ is the most computationally expensive layer in LPCNet. (3) The model footprint becomes large because of the embedding tables corresponding to the feedback samples.

To overcome these problems, we improved the Bunched LPCNet architecture with the three methods described in Section~\ref{section:proposed}.




%jh {첫 문단 마지막 bit bunching 간단히 설명하는 문장에서 output bit가 두 개로 나뉘어서 각각 higher bit, lower bit를 예측한다는 문장이 추가되면 어떨까요? ex) by splitting the (each?) output bit into 2 bits, the one for higher bit (coarse prediction) and the other for lower bit (fine correction)} -> sj: 조금 바꾸어서 반영했습니다. 의견 감사합니다.





==> BunchedLPCNet2_INTERSPEECH2022 (Version 4313)/conclusion.tex <==
\label{section:conclusion}
We introduced Bunched LPCNet2, which is a highly efficient neural vocoder architecture, and some presets to provide high-fidelity real-time TTS service to satisfy various device specifications, as confirmed by the MOS tests and RTF evaluations. We also investigated a simple technique that can significantly reduce the model size without degrading the speech quality. Compared with our previous study~\cite{bunched}, \textit{B-LPCNet2-R} achieved better speech quality and lower complexity with a model size of only 1.1 MB. In terms of quality, complexity, and model footprint, Bunched LPCNet2 would be the best candidate for low-resource edge devices, such as smart watches, wireless earphones, and home assistant devices.

==> BunchedLPCNet2_INTERSPEECH2022 (Version 4313)/experiments.tex <==
\label{section:evaluation}
\subsection{Experimental environment}
The several combinations of hyper parameters were chosen empirically to satisfy various device specifications as summarized in Table~\ref{tab:systems}, compared with Bunched LPCNet. We attempted to control the complexity of the models using $S$ and $n_{a}$ and determined an output layer to efficiently work for a given model capacity. For example, \textit{B-LPCNet2-R} was chosen because the SL layer is more efficient than the softmax layer where $S=2$ and $n_{a}=224$ in Figure~\ref{fig:mcd}. In addition, the temperature parameter $T$ was adjusted to suppress the noise generated by the low-complexity models. Finally, the \textit{B-LPCNet2-L}, \textit{B-LPCNet2-R}, and \textit{B-LPCNet2-S} target cloud, high-end, and low-end devices, respectively, and \textit{B-LPCNet2-S16} was prepared for low-resource devices that need to lower the  sampling rate. The other hyperparameters were set identically to~\cite{bunched}.

A Tacotron variant architecture~\cite{lpctron} was employed as a prosody model to evaluate the speech quality in the TTS pipeline. The systems were trained using two datasets: one of a professional English male speaker (17-hours with 10,000 utterances) and another of a professional English female speaker (15-hours with 7,612 utterances). Each vocoder model and prosody model were trained with a single speaker. Sixty utterances were used as a test set, and one percent of the remaining utterances were used as the validation set for training.

\subsection{Performance}
For the quality evaluation, we conducted mean opinion score (MOS) tests~\cite{itu-t} on the Amazon Mechanical Turk platform with 300 people and 120 unseen test utterances. For the complexity evaluation, we measured the RTF (Real Time Factor) on two devices: 1) an AWS c5.4xlarge instance (Intel Xeon Platinum 8124M CPU @ 3.00GHz) with Ubuntu 18.04 - representing a cloud device and 2) a Raspberry Pi (RPi) 3B v1.2 (BCM2837 @ 1.20 GHz) with Tizen 6.5 - representing an edge device. Our implementation was optimized using SIMD (Single Instruction Multiple Data) with single thread for each architecture. To demonstrate that our systems are as efficient as conventional vocoders, we also measured the complexity of the WORLD vocoder~\cite{world}\footnote{An open source code at \url{https://github.com/mmorise/World} was used }. Table~\ref{tab:mos} presents the evaluation results.

\begin{table}[t]
	\caption{MOS with 95\% confidence intervals and real time factor on each CPU architecture}
	\label{tab:mos}
	\centering
	\begin{tabular}{ c|ccc }
		\toprule
     	\multirow{2}{*}{\textbf{Systems}} &
		\multirow{2}{*}{\textbf{MOS}} &
		\multicolumn{2}{c}{\textbf{RTF}} \\
		& & \textbf{Intel Xeon} & \textbf{RPi} \\
     	\midrule
		\textit{Original(24kHz)} & $4.51 \pm0.04$ & - & - \\
		\textit{Original(16kHz)} & $4.12 \pm0.05$ & - & -\\
		\midrule
		\textit{B-LPCNet} & $3.95 \pm0.06$ & 0.072 & 2.394 \\
		\midrule
		\textit{B-LPCNet2-L} & $4.08 \pm0.06$ & 0.137 & 5.538 \\
		\textit{B-LPCNet2-R} & $3.99 \pm0.06$ & 0.051 & 1.657 \\
		\textit{B-LPCNet2-S} & $3.90 \pm0.06$ & 0.030 & 0.720 \\
		\textit{B-LPCNet2-S16} & $3.81 \pm0.06$ & 0.021 & 0.507 \\
		\midrule
		\textit{WORLD} & - & 0.075 & 1.808 \\
		\bottomrule
	\end{tabular}
\end{table}


The \textit{B-LPCNet2} systems with an SL layer demonstrated a highly efficient performance. The \textit{B-LPCNet2-L} generated sufficiently high fidelity speech for cloud TTS. The \textit{B-LPCNet2-R} achieved a lower complexity than the \textit{B-LPCNet} and even the WORLD vocoder. The \textit{B-LPCNet2-S} and \textit{B-LPCNet2-S16} works 7.7x and 10.9x faster than the \textit{B-LPCNet2-L}, respectively, on the RPi while maintaining a satisfactory speech quality. Employing them with a lightweight prosody model, a real-time TTS system is deployable on low-resource edge devices.

\subsection{Model footprint}

To investigate the efficiency in terms of the model footprint, we compared the MOS results to the model size. Notably, the separated format in Section~\ref{subsec:embed} is applied to all evaluated systems, and the model size included file headers less than 1 KB. Table~\ref{tab:footprint} summarize the results.

\begin{table}[h]
	\caption{MOS with 95\% confidence intervals and the model footprint for different embedding dimensions}
	\label{tab:footprint}
	\centering
	\begin{tabular}{ l|ccc }
		\toprule
		\multicolumn{1}{c|}{\textbf{Systems}} & \textbf{MOS} & \textbf{Model Size} \\
     	\midrule
     	\textit{B-LPCNet} & $3.95 \pm0.06$ & 10.141 MB \\
     	\midrule
     	\textit{B-LPCNet2-L} & $4.08 \pm0.06$ & 1.136 MB \\
     	~└ $n_{e}=128$ & $4.07 \pm0.06$ & 3.496 MB \\
     	\midrule
     	\textit{B-LPCNet2-R} & $3.99 \pm0.06$ & 1.135 MB \\
     	~└ $n_{e}=128$ & $3.97 \pm0.06$ & 3.834 MB \\
     	\midrule
     	\textit{B-LPCNet2-S} & $3.90 \pm0.06$ & 1.099 MB \\
     	~└ $n_{e}=128$ & $3.87 \pm0.06$ & 4.898 MB \\
     	\midrule
     	\textit{B-LPCNet2-S16} & $3.81 \pm0.06$ & 1.071 MB \\
		\bottomrule
	\end{tabular}
\end{table}

The systems with $n_{e}=128$, including \textit{B-LPCNet}, has a relatively large number of parameters. This results from the model size of Bunched LPCNet highly depending on the bunch size, embedding dimension, and $\text{GRU}_{\text{A}}$ units, as mentioned in Section ~\ref{subsec:embed}. In contrast, the \textit{B-LPCNet2} architectures show significantly small footprints of approximately 1.1 MB. Indeed, without the separated format, the size of the \textit{B-LPCNet} is 15.4 MB. Compared to the original Bunched LPCNet, this means that the \textit{B-LPCNet2-R} generates higher speech quality with only 7\% of the parameters.

To confirm the effect of the embedding dimension $n_{e}$ on speech quality, we also compared the MOS results for $n_{e}=1$ and $n_{e}=128$. We expected that the speech quality would degrade considerably, but the quality difference is negligible.

Figure~\ref{fig:embed} illustrates the trained embedding values of \textit{B-LPCNet2-S}. Note that the horizontal lines at both ends arose from our optimization trick that maps the sparse indices to the adjacent dense index, preventing access to untrained weights in inference. Each line has a different scale, slope, symmetrical point, and nonlinearity. This suggests that the trained embedding table with $n_{e}=1$ controls the nonlinear transforms with desirable properties from the network. Evidently, this is more outstanding than directly feedbacking the scalar value.

\begin{figure}[h]
\centering
\includegraphics[width=0.4\textwidth]{figures/embed.pdf}
\caption{The plot of trained embedding value with $n_{e}=1$.\\\hspace{\textwidth}(A total of 30 lines = 2 speakers $\cdot$ 3 feedback samples $\cdot$ 5 Sample Bunching)}
\label{fig:embed}
\end{figure}






==> BunchedLPCNet2_INTERSPEECH2022 (Version 4313)/introduction.tex <==
% Related Works.


%- 니즈 : TTS를 활용처가 많이 늘어나 있다. 대부분의 TTS 서비스는 Cloud 기반 TTS로 서버기반의 GPU, CPU를 활용하는 형태로 서비스 되고 있다. 그런데, 이러한 서버 기반의 서비스는 privacy 이슈에서 자유로울 수가 없기 때문에, 디바이스에서만 동작되는 TTS에 대한 니즈가 생기고 있다. 그런데, 디바이스는 예를 들어 smart phone과 같은 고성능의 cpu를 포함하고 있는 device들도 있으나, smart watch, ear-buds 등과 같은 저사양의 device들도 있다. 이러한 다양한 resource의 device에서 연산량-음질간의 trade off를 효율적으로 control 하여, 서비스를 제공할 수 있는 문제가 대두되고 있다~\cite{wu2020fbwave}.
%LPCNet~\cite{valin-lpcnet} is a state-of-the-art light-weight vocoder which is operating on CPU efficiently with keeping high speech quality. In the Bunched LPCNet\cite{bunched}, we have introduced Sample Bunching and Bit Bunching techniques to reduce computational cost with keeping high speech quality and also shown the possibility of the LPCNet on operating in wide coverage from the cloud server to the low-end mobile devices. The Bunching techniques in \cite{bunched} is a smart way to generate multiple samples with sharing higher cost layers. However, it has limitation where complexity reduction factor is saturated from bunch size 4. And also huge quality drop cannot be avoidable, when trying to reduce number of GRU units based on the Bunching techniques. In order to extending the coverage of the Bunched LPCNet, very low-resource device needs to be attended.

Nowadays, as many types of edge devices emerge, people utilize text-to-speech (TTS) services in their daily life without device-constraints. Although most TTS systems now have been launched on cloud servers, running on edge devices resolves significant concerns, such as latency, privacy, and internet connectivity issues. Note that edge devices include high-resource devices, such as smartphones, and low-resource devices, such as smart watches, wireless earphones, and home assistant devices. To deploy TTS services on these devices optimizing the performance within a given resource is crucial. Additionally, expanding the service capability while maintaining the architecture is worthwhile instead of developing new architectures for specific devices. For this purpose, FBWave~\cite{wu2020fbwave} proposed a flow-based scalable vocoder architecture to easily control the computational cost. However, it demonstrated an insufficient speech quality in cloud servers, even in high-quality mode. This study introduces a vocoder family that can provide a wide coverage on computational cost constraints from cloud to low-resource edge devices.

%Text-to-speech (TTS) is one of essential components in voice interface to deliver information to users. Nowadays, more advanced features not only delivering information are requested from commercial fields, e.g., various styles to give fun to users, bi(multi)-lingual capability to fluent conversation with foreigners, on-device TTS on even very low-resource edge devices such as smart watches, wireless earphones and so on. Since most TTS services now have been launched based on cloud server, extending the service capability with keeping TTS architectures is worthwhile instead of developing new TTS architectures for the specific purpose~\cite{wu2020fbwave}. Current state-of-the-art neural TTS models are consisting of grapheme to phoneme to convert an utterance to phoneme sequences, prosody model to predict acoustic features from phoneme sequences and finally vocoder to generate speech waveform from the acoustic feature sequences. The Vocoder is normally bottleneck in terms of computational cost ~\cite{wu2020fbwave,bunched} and this paper is focusing on vocoder family which is able to providing wide coverage on computational cost constraints.

Many neural vocoders have been proposed since WaveNet, which predicts a waveform directly, was presented~\cite{oord2016wavenet}. Early neural vocoders are based on a computationally expensive auto-regressive (AR) manner~\cite{oord2016wavenet,kalchbrenner2018efficient}, impractical for real-time services. Inferring in parallel on GPUs have also been attempted~\cite{prenger2019waveglow,kumar2019melgan,kong2020hifi}, but few edge devices have a GPU.
On the other hand, LPCNet~\cite{valin-lpcnet} is a light-weight vocoder based on AR architecture that is suitable for on-device inference. To the best of our knowledge, LPCNet is still one of the best candidates that can efficiently generate speech on a CPU, even with a high quality. Many LPCNet variants have been introduced: iLPCNet~\cite{hwang2020improving} and Full-Band LPCNet~\cite{matsubara2021full} were studied to improve speech quality; and Bunched LPCNet~\cite{bunched}, Gaussian LPCNet~\cite{popov2020gaussian}, and Sub-band LPCNet~\cite{cui2020efficient} were studied to reduce complexity without sacrificing speech quality. However, the variants are unsatisfactory for low-resource edge devices in that they target high-end devices, such as smart phones. A quality drop is also observed by shrinking the network capacity for low-resource devices.

%to push it operating on the extreme low-resource devices with keeping their own design philosophies.

%There have been proposed many vocoders, since the WaveNet was proposed to generate waveform directly from linguistic features. Most of the neural vocoders are modeling speech waveform, i.e. WaveNet~\cite{oord2016wavenet}, WaveRNN~\cite{kalchbrenner2018efficient}, WaveGlow~\cite{prenger2019waveglow}, MelGAN~\cite{kumar2019melgan}, and  Hifi-GAN~\cite{kong2020hifi} by using CNN architectures or RNN with AR or non-AR models and it is assumed that those vocoders are serviced by GPU. On the other hand, utilizing speech productive model, i.e. source-filter model\cite{sound-principles}, in LPCNet~\cite{valin-lpcnet} combination of modeling vocal tract by signal processing and modeling excitation probability distribution by neural network can achieve high quality speech and high efficient generation by CPU together. To the best of our knowledge, LPCNet is still one of the best performed ones which can infer speech efficiently and even more high quality speech on CPU. There have been many variants in LPCNet, iLPCNet~\cite{hwang2020improving} and Full-Band LPCNet~\cite{matsubara2021full} studied to improve the speech quality of LPCNet and Bunched LPCNet~\cite{bunched}, Gaussian LPCNet~\cite{popov2020gaussian}, Subband LPCNet~\cite{cui2020efficient} studied to reduce the cost of operation without sacrificing speech quality. The latter LPCNet variants are basically designed to share the high cost layers, i.e. GRU layers, on generating multiple samples. However, the variants are not suitable to the very low-end edge devices in that they were developed focusing on smart phones and then quality drop can be easily observed to push it operating on the extreme low-resource devices with keeping their own design philosophies.

In this paper, we introduces Bunched LPCNet2, which is an improved Bunched LPCNet that addresses the problems arising when covering a wide range of devices, from cloud servers to wearable devices such as smart watches and AR/VR glasses. Our contributions include three methods:
%when it is tried to cover wide range devices from cloud servers to wearable devices like smart watches and AR/VR glasses efficiently by the Bunched LPCNet Family. Our contributions include three methods:

\begin{enumerate}
\item Single logistic output layer that extends the coverage of Bunched LPCNet to low-resource constraints.
\item Dual-rate LPCNet for computational and maintenance cost reduction.
\item Insightful tricks that significantly reduce the model footprint.
\end{enumerate}

We present a brief overview of Bunched LPCNet in Section~\ref{section:bunched}, followed by an in-depth description of the proposed methods in Section~\ref{section:proposed}. Section~\ref{section:evaluation} summarizes the evaluation results in terms of computational cost and speech quality. Finally, Section~\ref{section:conclusion} concludes the paper.

%Our previous works.

%Sample bunching과 Bit bunching은 Layer unit을 줄이는 방법보다 효과적임. 하지만, Output layer의 연산량으로 인해 Sample bunch size 4 이상에서는 연산량 감소효과가 작다. 더 많은 연산량 감소를 위해서는 GRU unit을 줄여야하는데, 그럴경우 성능이 크게 감소한다. 게다가 Sample bunch size가 늘어날 경우, Sample Embedding table의 크기가 비례하여 증가하므로, 모델 크기가 커진다. 이 논문에서는 On-device에 적합한 Neural Vocoder를 위하여, 낮은 연산량과 작은 모델크기에서도 음질 저하를 최소화할 수 있도록 아래 항목들을 제안함.

%\begin{enumerate}
%\item LPCNet의 GRU unit 감소에 따른 음질저하를 최소화하고, Output layer 및 Sampling 연산량을 감소할 수 있는 Single logistic layer
%\item 모델 크기를 significantly 감소가능한 Sample embedding table dump 방법.
%\item Sampling rate를 낮춤으로써 연산량 감소가 가능한 Dualrate 구조.
%\end{enumerate}

%jh{source-filter model 언급 부분에 해당 개념 다룬 논문 인용하는 건 어떨까요? (The Vowel, its Nature and Structure, 1953); Bunched LPCNet에선 해당 논문 인용했더라고요} -> %kh{네, 맞네요.반영하려고 하니, 1941년 문헌이 적혀 있네요.. 검색이 잘 안되는데.. } -> jh{41년 문헌이 맞는 것 같습니다. 제가 잘못 파악했었네요..}
%jh{Intro 마지막 문단 'followed by in-depth description on our proposed architecture in Section 3' 이 문장에서 proposed architecture 대신 proposed methods는 어떨까요?} -> %kh{반영했어요. 감사합니다.}



==> BunchedLPCNet2_INTERSPEECH2022 (Version 4313)/proposed.tex <==
\label{section:proposed}
\subsection{Single logistic output layer}
\label{subsec:sl}

\begin{figure}[b]
    \centering
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/comp_mcd_rnn.pdf}
        \caption{on $\text{GRU}_{\text{A}}$ units ($S$=1) }
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/comp_mcd_bunch.pdf}
        \caption{on bunch size ($n_{a}$=384)}
    \end{subfigure}
    \hfill
    \caption{MCD plots of softmax and single logistic output layer}
    \label{fig:mcd}
\end{figure}

Auto-regressive vocoders generate waveforms by sampling from the probability density function with non-parametric or parametric distributions. Non-parametric methods, e.g., a softmax output layer, can model complex distributions and show a good performance in modeling waveforms~\cite{oord2016wavenet, valin-lpcnet}, but the computations in the output layer and sampling process from a categorical distribution are expensive by a large output dimension; for example, 256 for an 8-bits $\mu$-law quantization~\cite{mulaw-quantization}. Additionally, its speech quality is significantly degraded when the model has insufficient capacity.

Accordingly, we attempted to employ parametric distributions based on previous studies~\cite{tacotron2,pmlr-v80-oord18a}, which used a mixture of logistics (MoL) as an output distribution, and determined that a logistic output layer, particularly with single mixture, is a good alternative in terms of efficiency. To demonstrate the efficiency of the logistic layer in complexity reduction, we compare the mel-cepstral distances (MCD)~\cite{mcd} of single logistic (SL) to the softmax output layer with the smaller bunch size $S$ and $\text{GRU}_{\text{A}}$ units $n_{a}$ in Figure~\ref{fig:mcd}. Note that $S=1$ and $n_{a}=384$ correspond to the original LPCNet. As the model capacity decreases, the SL layers work more efficiently than the softmax layers. We believe that a non-parametric loss could lead the network to predict complex distributions beyond the model capacity. That is, it could cause an under-fitting problem when the model capacity is too small. In contrast, a unimodal parametric distribution simplifies an objective and lowers the training difficulty by reducing the burden on the network. It can mitigate the quality reduction despite an insufficient capacity. 

Figure~\ref{fig:sl} presents our network architecture for the SL layer. The FC block comprises fully-connected (FC) layers with 16 units, and the output dimension of a final FC layer is 2. A location parameter $\mu_{t}$ and scale parameter $s_{t}$ are obtained from the custom activation functions $\alpha 1$ and $\alpha 2$ as follows.
\begin{align}
    \label{eq1}
    \mu_{t} &= \alpha 1(h_{t,1}) = \tanh{(h_{t,1}/u)} \\
    \label{eq2}
    s_{t} &= \alpha 2(h_{t,2}) = \exp{(\tanh{(h_{t,2})} \cdot v - w)}
\end{align}
$u$, $v$, and $w$ help maintain the training stable, and are set empirically, to 64, 16 and 6, respectively. The model is trained to maximize the discretized logistic likelihood~\cite{pixelcnn} on normalized 16-bit samples from -1 to +1. Finally, $\hat{e}_{t}$ is sampled from the logistic distribution, as defined in (\ref{eq3}).
\begin{equation}
    \hat{e}_{t} = \mu_{t} + T \cdot s_{t} \cdot \ln(\epsilon/(1-\epsilon)), \quad \epsilon \sim \text{Uniform}(0,1)
    \label{eq3}
\end{equation}
where $T$ denotes a temperature parameter. When $\hat{e}_{t}$ is fed to the embedding tables, the 8-bit $\mu$-law quantization is applied.

Employing the deep and narrow layers, the proposed architecture demonstrates a better performance while satisfying a lower complexity than the softmax layer. Moreover, the sampling process of the SL layer is undoubtedly simple and computationally cheap using only scalar operations.

%- 모델 Capacity가 큰 경우에는 Non-parametric distribution(e.g. softmax)이나 Parametric multi-modal distribution(e.g. GMM and MoL)이 우수한 성능을 보인다. 하지만 제한된 Capacity에서는 Unimodal distribution이 우수함. 그 중에서 우리는 Sampling이 빠른 Single logistic(SL) output layer를 선택함.
%- Softmax / MoL / SL 에서 Bunching 사이즈에 따른 음질 변화 데이터.
%- DualFC + softmax 대신 Dense Layer + SL 구조 설명. Softmax의 출력차원 256을 감소시킬 수 있음.
%- Loss 정의 + Scaling 효과(16을 곱하고 6으로 빼주는 과정)
%- Sampling 방법 + Softmax 대비 연산량 우수함. Sampling temperature 언급. 모델이 작아지면서 Noise 발생시 temperature를 조절하여 Noise를 감쇄시킬 수 있음.
%- Feedback 시 mulaw quantization 적용  \textbf{이부분은 3.2로 옮기는 것이 어떨까요?} \textbf{네. 그것도 좋은 방법 같습니다. 3.1부터 작성 후 어느곳이 적절한지 결정해보겠습니다.}

\begin{figure}[t]
\centering
\includegraphics[width=0.25\textwidth]{figures/sl2.pdf}
\caption{Network architecture for single logistic output layer}
\label{fig:sl}
\end{figure}

\begin{table*}[t]
	\caption{System Configurations}
	\label{tab:systems}
	\centering
	\begin{tabular}{ c|ccccccc }
		\toprule
		\textbf{Systems} & \textbf{Output Layer} & $\bm{S}$ & $\bm{n_{a}}$ & $\bm{n_{e}}$ & $T$ & \textbf{Sampling rate} & \textbf{Target device}\\
		\midrule
		\textit{B-LPCNet}\cite{bunched} & Softmax with Bit Bunching & 4 & 384 & 128 & 0.75 & 24 kHz & High-end \\
		\midrule
		\textit{B-LPCNet2-L} & Softmax & 1 & 384 & 1 & 0.75 & 24 kHz & Cloud \\
		\textit{B-LPCNet2-R} & Single logistic & 2 & 224 & 1 & 0.75 & 24 kHz & High-end \\
		\textit{B-LPCNet2-S} & Single logistic & 5 & 176 & 1 & 0.65 & 24 kHz & Low-end \\
		\textit{B-LPCNet2-S16} & Single logistic & 5 & 176 & 1 & 0.65 & 16 kHz & Low-end \\
		\bottomrule
	\end{tabular}
\end{table*}

\subsection{DualRate LPCNet}
\label{subsec:dualrate}


For low-resource devices, a more compact model would be required. However, a model with low capacity inevitably generates annoying sounds, e.g., noisy or muffled sounds. Reducing the sampling rate could be a solution of this problem.

By the way, a prosody model of a TTS system requires continuous maintenance, even after deployed, so that the pronunciation errors or unnatural prosody for given texts can be fixed. In other words, employing an additional prosody model for a low sampling rate vocoder leads to a maintenance cost increase. For this reason, we propose a DualRate LPCNet, which is an architecture that provides two sampling rates (24 kHz and 16 kHz) from one prosody model, as depicted in Figure~\ref{fig:dualrate}. Note that $x_{i}$ and $F_{i}$ denote the $i$ kHz waveform and acoustic features extracted from $x_{i}$, respectively.

The feature conversion block computes $F'_{16}$, which is the input of 16 kHz LPCNet, to remove unnecessary information from $F_{24}$ and obtain higher mutual information with a target $x_{16}$.
The acoustic features $F_{24}$, which comprise 20 cepstral coefficients, a pitch period, and a pitch correlation, are converted as follows.
\begin{itemize}
    \item The 20 cepstral coefficients are extracted with 20 CELT bands from the Opus codec~\cite{opus}. The 20 CELT bands cover up to a 12 kHz bandwidth, and the last two bands cover from 8 kHz to 12 kHz. The two unnecessary bands are removed by sequentially computing the IDCT, low-pass filter, and DCT. Finally, the 18 cepstral coefficients that cover up to an 8 kHz bandwidth are obtainable.
    \item The pitch period is multiplied by the ratio of sampling rates $(\frac{16k}{24k}=\frac{2}{3})$.
    \item The pitch correlation is used as is.
\end{itemize}
Using the 16 kHz LPCNet trained with the converted $F'_{16}$, we can save on both computational and maintenance costs. Similarly, the TTS systems for given devices can be easily deployed by choosing suitable LPCNet models with various complexities.

%\tobefixed{Furthermore, if the LPCNet models with various computational costs are prepared, TTS systems can be easily deployed by choosing a suitable LPCNet model for various device specifications.}

\subsection{Optimizing model footprint}
\label{subsec:embed}
%\sj{Need to change the subsection title. Candidate 1) Optimizing model footprint }

\begin{figure}[b!]
\centering
\includegraphics[width=0.48\textwidth]{figures/dualrate2.pdf}
\caption{Training / inference procedure of DualRate LPCNet.}
\label{fig:dualrate}
\end{figure}

Although Sample Bunching has an efficient architecture for reducing the computational complexity, it increases the number of model parameters by the embedding tables corresponding to the feedback samples $X$, where $\bm{X}=\{\hat{p}_{t-S+1}:\hat{p}_{t}, \hat{x}_{t-S}:\hat{x}_{t-1},\hat{e}_{t-S}:\hat{e}_{t-1} \}$, as depicted in Figure~\ref{fig:bunched}. As mentioned in~\cite{bunched}, $E_{x \in \bm{X}}$ is converted into a pre-computed lookup table $E'_{x}$ obtained from the multiplication of $E_{x}$ and $U_{x}$, the input weight matrix in $\text{GRU}_{\text{A}}$, to replace matrix-vector multiplication operations with vector-vector addition operations. Specifically, $E_{x}$ with a $[2^{8}, n_{e}]$ shape is converted to $E'_{x}$ with a $[2^{8}, 3 \cdot n_{a}]$ shape, where $n_{e}$ and $n_{a}$ denote the embedding dimension of $E_{x}$ and number of $\text{GRU}_{\text{A}}$ units, respectively. The total number of parameters in $E'_{x}$ is $2^{8} \cdot 3 \cdot n_{a} \cdot (3 \cdot S)$. With the default hyperparameters of Bunched LPCNet, $n_{e}=128$ and $n_{a}=384$, their parameters account for 70\% of the model, even when $S=1$. Therefore, we focus on reducing the embedding table size.

To optimize the model footprint, we attempted to feedback the scalar values into $\text{GRU}_{\text{A}}$. The first method worth considering is to feedback the scalar values directly without the embedding table. However, this wastes the model capacity to transform the scalar values into the desired representation from the network. To feedback desired values into the network without wasting model capacity, a nonlinear mapping function from a quantized value to a continuous value would be useful, which is the embedding table with $n_{e}=1$. This could degrade the speech quality compared to when $n_{e}=128$. However, we determined that it has a small effect on the performance, whereas the size of $E_{x}$ and $U_{x}$ can be significantly reduced.

Note that $n_{e}$ does not affect the size of the dumped model owing to $E'_{x}$ with the fixed shape $[2^{8}, 3 \cdot n_{a}]$ being independent from $n_{e}$. Thus, we dumped $E_{x}$ with the $[2^{8}, n_{e}]$ shape and $U_{x}$ with the $[n_{e}, 3 \cdot n_{a}]$ shape separately into a model instead of $E'_{x}$ (hereafter referred to as separated format). Note that it works only when $2^{8} \cdot n_{e} + n_{e} \cdot 3 \cdot n_{a} < 2^{8} \cdot 3 \cdot n_{a}$. For example, when $n_{e}=128$, $n_{a}$ must be greater than 85. The greater $n_{a}$ and the less $n_{e}$ achieve the higher reduction ratio. The total number of parameters is reduced to $(2^{8} \cdot n_{e} + n_{e} \cdot 3 \cdot n_{a} ) \cdot (3 \cdot S)$ without performance degradation. $E'_{x}$ can be restored during inference engine initialization. The separated format facilitates an extremely small model footprint: 70\% reduction for $S=1$ and 82\% reduction for $S=2$ when $n_{e}=1$ and $n_{a}=384$.

%When $n_{e}=1$ and $n_{a}=384$, with the separated format, the total model parameters can be reduced by 70\% for $S=1$, and by 82\% for $S=2$.

%1) embed_size 크기를 줄이기 위해 scalar 값을 feedback하는 방법 사용.
%2) 하지만, quantized value를 scalar로 feedback할 경우, 표현력에 문제가 있음. scalar 값에서 모델이 필요한 정보를 뽑아내기 위해 모델 capacity가 낭비됨.
%3) 그래서 크기가 1인 embed_size를 사용하기로 함. 아래의 장점을 가짐.
%  - embed_table 크기가 작기때문에, 모델 크기를 유지할 수 잇음. (~수KB)
%  - 추가 연산량 없이 높은 non-linear 변환 가능. 크기 1의 embedding table은 discrete value를 continous value로 바꿔주는 mapping function으로써 동작하며, 모델이 필요한 정보로 미리 변환하여 feedback 해주기 때문에, 단순히 PCM value를 feedback하는 것보다 더 효율적으로 동작할 수 있음.

%introduce two simple methods which can make the embedding table extremely small.

%To optimize model footprint, we introduce two simple methods which can make the embedding table extremely small.
%\begin{itemize}
%    \item \textbf{Method 1:} Dump $E_{x}$ and $U_{x}$ separately into a model instead of $E'_{x}$; Note that it works only when $2^{8} \cdot n_{e} + n_{e} \cdot 3 \cdot n_{a} < 2^{8} \cdot 3 \cdot n_{a}$. For example, when $n_{e}=128$, $n_{a}$ needs to be greater than 85. The total number of parameters can be reduced to $(2^{8} \cdot n_{e} + n_{e} \cdot 3 \cdot n_{a} ) \cdot (3 \cdot S)$ without performance degradation. $E'_{x}$ can be restored during inference engine initialization.
%    \item \textbf{Method 2:} Feedback scalar values with $n_{e}=1$; It could degrade the speech quality. However, we found that it has very small effect on the performance, whereas the size of $E_{x}$ and $U_{x}$ can be reduced significantly. \tobefixed{Add some analysis}
%\end{itemize}

%Consequently, the total model parameters can be reduced by 70\% for $S=1$, and by 82\% for $S=2$.

% When S=1, 4.808MB -> 1.450 MB
% 실제 훈련한 weight plot. log scale처럼 출력되는 것 확인. + plot 분석? 자리 남으면 추가!
% model 크기 비교할때 REDUCED\_CKPT\_FORMAT은 전부다 켜놓으려고해요.

%jh{Single Logistic 설명 부분에 MoL 적용한 TTS 논문 reference? ; Parallel Wavenet or Tacotron2} -> sj: 좋은 의견이십니다. 일단 현재 텍스트에서 적당히 달 수 있는 곳이 없어서 텍스트를 좀 바꿔볼지 고민해보겠습니다.
%jh{MCD; 관련 논문 인용? Mel-cepstral distance measure for objective speech quality assessment (1993)} -> sj: 추가했습니다.

%kh{Figure 2(b)에서 $n_{a}$=384 가 있어야 할거 같네요. --> Figure subtitle에 반영했습니다.}

%kh{"the computations in the output layer and sampling process from a categorical distribution are slow  --> slow 대신에 expensive로 바꾸는 것이 좋을것 같아서 반영했습니.} sj: 확인했습니다. 감사합니다.


